Quantum Circuit Reconstruction from Power Side-Channel Attacks on Quantum Computer Controllers

The interest in quantum computing has grown rapidly in recent years, and with it grows the importance of securing quantum circuits. A novel type of threat to quantum circuits that dedicated attackers could launch are power trace attacks. To address this threat, this paper presents first formalization and demonstration of using power traces to unlock and steal quantum circuit secrets. With access to power traces, attackers can recover information about the control pulses sent to quantum computers. From the control pulses, the gate level description of the circuits, and eventually the secret algorithms can be reverse engineered. This work demonstrates how and what information could be recovered. This work uses algebraic reconstruction from power traces to realize two new types of single trace attacks: per-channel and total power attacks. The former attack relies on per-channel measurements to perform a brute-force attack to reconstruct the quantum circuits. The latter attack performs a single-trace attack using Mixed-Integer Linear Programming optimization. Through the use of algebraic reconstruction, this work demonstrates that quantum circuit secrets can be stolen with high accuracy. Evaluation on 32 real benchmark quantum circuits shows that our technique is highly effective at reconstructing quantum circuits. The findings not only show the veracity of the potential attacks, but also the need to develop new means to protect quantum circuits from power trace attacks. Throughout this work real control pulse information from real quantum computers is used to demonstrate potential attacks based on simulation of collection of power traces.

==> sections/background_dist.tex <==
\subsubsection{Divergences, Distances and Metrics}\label{sec::divergences}
In per-channel single trace attacks, we use the Kullback-Leibler divergence (KLD) and the Jensen-Shannon divergence (JSD) and its distance ($\sqrt{\text{JSD}}$) to distinguish two probability distributions. Therefore, here we provide a brief introduction to divergences, distances and metrics. For more details, we refer the reader to~\cite{deza2009encyclopedia, hayashi2014introduction}.
%
A \textit{metric} $d$ on a set $\chi$ is a function $d: \chi \times \chi \rightarrow \mathbb{R}_{\geq 0}$ such that for any $x, y, z \in \chi$ the following properties are satisfied:
\begin{align}
  d(x, y) & \geq 0 \label{non-negativity}\tag{non-negativity}                                                 \\
  d(x, y) & =0 \text{ if and only if } x=y \label{idendity-of-indiscernibles}\tag{identity of indiscernibles} \\
  d(x, y) & =d(y, x) \label{symmetry}\tag{symmetry}                                                           \\
  d(x, y) & \leq d(x, z)+d(z, y) \label{triangle-inequality}\tag{triangle inequality}
\end{align}
$\chi$ represents the set of probability distributions and $x$ or $y$ represent an entire probability distribution such as $P=\left\{p_1, p_2, \ldots, p_n\right\}$ where $p_i \geq 0$ and $\forall i, \sum_{i=1}^n p_i=1$. Often, if a distance measure $d$ only satisfies the property~\ref{non-negativity}, is called a \textit{divergence}. If, in addition, $d$ satisfies the properties \ref{idendity-of-indiscernibles}, and \ref{symmetry}, it is called a \textit{distance}.


==> sections/benchmark-full.tex <==
\begin{table*}[h]
  \centering
  % \footnotesize 
  \scriptsize
  \caption{QASMBench Benchmark Suite version 1.4~\cite{qasmbench}}
  \label{tab:benchmarks}
  \begin{tabular}{@{}llccccc@{}}
    \toprule
    {\bf Benchmark}     & {\bf Description}                             & {\bf Algorithm}         & {\bf Qubits} & {\bf Gates} & {\bf CX} & {\bf Ref}            \\ \midrule
    deutsch             & Deutsch algorithm with 2 qubits for f(x) = x  & Hidden Subgroup         & 2            & 5           & 1        & \cite{openqasm}      \\
    iswap               & An entangling swapping gate                   & Logical Operation       & 2            & 9           & 2        & \cite{openqasm}      \\
    quantumwalks        & Quantum walks on graphs with up to 4 nodes    & Quantum Walk            & 2            & 11          & 3        & \cite{quantumwalks}  \\
    grover              & Grover's algorithm                            & Search/Optimization     & 2            & 16          & 2        & \cite{agent_anakin}  \\
    ipea                & Iterative phase estimation algorithm          & Hidden Subgroup         & 2            & 68          & 30       & \cite{openqasm}      \\
    dnn                 & 3 layer quantum neural network sample         & Machine Learning        & 2            & 226         & 42       & \cite{dnn}           \\
    \midrule
    teleportation       & Quantum teleportation                         & Quantum Communication   & 3            & 8           & 2        & \cite{teleportation} \\
    qaoa                & Quantum approximate optimization algorithm    & Search/Optimization     & 3            & 15          & 6        & \cite{qaoa}          \\
    toffoli             & Toffoli gate                                  & Logical Operation       & 3            & 18          & 6        & \cite{scaffold}      \\
    linearsolver        & Solver for a linear equation of one qubit     & Linear Equation         & 3            & 19          & 4        & \cite{linearsolver}  \\
    fredkin             & Controlled-swap gate                          & Logical Operation       & 3            & 19          & 8        & \cite{scaffold}      \\
    wstate              & W-state preparation and assessment            & Logical Operation       & 3            & 30          & 9        & \cite{openqasm}      \\
    basis\_change       & Transform the single-particle basis           & Quantum Simulation      & 3            & 53          & 10       & \cite{openfermion}   \\
    \midrule
    qrng                & Quantum random number generator               & Quantum Arithmetic      & 4            & 4           & 0        & \cite{qrng}          \\
    cat\_state          & Coherent superposition of two coherent states & Logical Operation       & 4            & 4           & 3        & \cite{scaffold}      \\
    inverseqft          & exact inversion of quantum Fourier tranform   & Hidden Subgroup         & 4            & 8           & 0        & \cite{openqasm}      \\
    adder               & Quantum ripple-carry adder                    & Quantum Arithmetic      & 4            & 23          & 10       & \cite{scaffold}      \\
    hs4                 & Hidden subgroup problem                       & Hidden Subgroup         & 4            & 28          & 4        & \cite{scaffold}      \\
    bell                & Circuit equivalent to Bell inequality test    & Logic Operation         & 4            & 33          & 7        & \cite{cirq}          \\
    qft                 & Quantum Fourier transform                     & Hidden Subgroupe        & 4            & 36          & 12       & \cite{openqasm}      \\
    variational         & Variational ansatz for a Jellium Hamiltonian  & Quantum Simulation      & 4            & 54          & 16       & \cite{openfermion}   \\
    vqe\_uccsd          & Variational quantum eigensolver with UCCSD    & Linear Equation         & 4            & 220         & 88       & \cite{scaffold}      \\
    basis\_trotter      & Trotter steps for molecule LiH at equilibrium & Quantum Simulation      & 4            & 1626        & 582      & \cite{openfermion}   \\
    \midrule
    qec\_sm             & Repetition code syndrome measurement          & Error Correction        & 5            & 5           & 4        & \cite{openqasm}      \\
    lpn                 & Learning parity with noise                    & Machine Learning        & 5            & 11          & 2        & \cite{sampaio96}     \\
    qec\_en             & Quantum repetition code encoder               & Error Correction        & 5            & 25          & 10       & \cite{sampaio96}     \\
    shor                & Shor's algorithm                              & Hidden Subgroup         & 5            & 64          & 30       & \cite{ibm_qiskit}    \\
    pea                 & Phase estimation algorithm                    & Hidden Subgroup         & 5            & 98          & 42       & \cite{openqasm}      \\
    error\_correctiond3 & Error correction with distance 3 and 5 qubits & Error Correction        & 5            & 114         & 49       & \cite{bench_2017}    \\
    \midrule
    simons              & Simon's algorithm                             & Hidden Subgroup         & 6            & 44          & 14       & \cite{agent_anakin}  \\
    qaoa                & Quantum approximate optimization algorithm    & Search and Optimization & 6            & 270         & 54       & \cite{cirq}          \\
    vqe\_uccsd          & Variational quantum eigensolver with UCCSD    & Linear Equation         & 6            & 2282        & 1052     & \cite{scaffold}      \\
    \midrule
    hhl                 & HHL algorithm to solve linear equations       & Linear Equation         & 7            & 689         & 196      & \cite{ibm_hhl}       \\
    \bottomrule
  \end{tabular}
\end{table*}



==> sections/calibration.tex <==
\subsection*{Todo: QC Calibration Evaluation}
--- For the amplitude of instructions: In the end, maybe we can have a figure, whose x axis is the time (date), and y axis is the standard deviation value. In the figure, each line is one native gate.However, because there are several backends, we may need to move this to appendices.  One way is to have one figure for each backend, but we may need to move this figure to appendices.  Another way is to have a table showing similar things as the figure, but it would still be big.

--- For the accuracy of the methods: Maybe we should first determine a list of circuits from the benchmarks which contain enough circuits, say 100 or more. Then compute the accuracy of recovering the correct circuits for each day. This may be similar to the above figure, except that now the y-axis is the accuracy, and we can pack all backends in one figure.


\begin{figure*}[h]
  \captionsetup[subfigure]{justification=centering}
  \centering
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/calibration-gates.png}
    \caption{Standard deviation of the amplitude of the native gates using the past calibration data.}
  \end{subfigure}%
  ~
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/accuracy-circuits.png}
    \caption{Accuracy of recovering the correct circuits using the past calibration data.}
  \end{subfigure}
  \caption{Calibration of Quantum Computers}
\end{figure*}

